The Intergalactic Medium

The intergalactic medium (IGM) comprises all the matter that lies between galaxies. Hosting the vast majority ($\gtrsim 90\%$) of the baryons in the Universe, the IGM is a critical reservoir and probe for cosmology and astrophysics, providing insights into large-scale structure formation and galaxy evolution. In this Chapter, we present an overview of the general properties of the IGM, focusing on their dependence on cosmic environment and cosmic time. Emphasis is given to the basic physical principles that allow us to model the density, temperature, and ionization state of the IGM, supported by results from cosmological hydrodynamical simulations. We also cover the foundational principles of quasar spectroscopy used to probe the IGM in absorption, with a particular focus on HI absorption lines. Finally, we briefly discuss future prospects and complementary observational techniques to enhance our understanding of the IGM.

==> figures/cosmic_web.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=.4\textwidth]{blankfig}
\includegraphics[width=.4\textwidth]{blankfig}
\caption{An slice of the cosmic web, from z=2 to z=0. The left panel shows dark matter while the right panel shows the baryons. Diffuse baryons in the IGM dominate this latter picture, as galaxies appear smaller than 1 pixel.}
\label{fig:lyaforest}
\end{figure}


==> figures/ionization_temperature.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.95\textwidth]{figures/ionization_temperature.png}
\caption{Left: Models and observational constraints for the IGM photoionization rates from the UVB ($\Gamma_{\rm HI}$) as a function of redshift. The models from \citet{khaire2019} (blue-solid line) and from \citet{haardt2012} (yellow-dashed line), among others, are shown. Figure from \citet{khaire2019}. Right: Models from and observations for the temperature of the IGM at mean density, $T_0$, as a function of redshift. Two models from \citet{upton2016} are shown: with (blue-solid line) and without (red-dashed line) \heii\ reionization. Figure adapted from \citet{upton2016}.}
\label{fig:ionization_temperature}
\end{figure}


==> figures/phase_diagram.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{figures/phase_diagram.png}
\includegraphics[width=0.45\textwidth]{figures/cen_ostriker.png}


\caption{Left: Density-temperature diagram for diffuse baryons at $z=0$ from a cosmological hydrodynamical simulation (Illustris TNG; \citealt{nelson2019}). The five phases presented in Section~\ref{sec:hydro} are labeled. Figure from \citet{galarraga2021}. Right: Volume (a) and Mass (b) fractions of the different gas phases as a function of redshift from the hydrodynamical simulation presented by \citet{cen2006}. Although the definition of the gas phases are slightly different than those presented in Section~\ref{sec:hydro}, this figure illustrates that the diffuse baryons (those outside galaxies) account for $\gtrsim 90$\,\% of the baryons in the Universe. At $z\gtrsim 2$, the dominant phase is the diffuse IGM (pink), whereas at $z\lesssim 0.5$ both the diffuse IGM and WHIM (red or black) dominate in almost equal proportion ($\sim 40$\,\%~each). The exact amount of baryons in the WHIM critically depends on galaxy feedback models. Here, a model with (red) and without (black) galactic winds are shown for reference. Figure from \citet{cen2006}.}
\label{fig:phase_diagram}
\end{figure}

